Newly observed $a_0(1817)$ as the scaling point of constructing the scalar meson spectroscopy

Stimulated by the newly observed $a_0(1817)$ by the BESIII Collaboration, we find a perfect Regge trajectory composed of the $a_0(980)$, $a_0(1450)$, and $a_0(1817)$, which leads us to categorize the $a_0(980)$, $a_0(1450)$, and $a_0(1817)$ into the isovector scalar meson family. This scenario is supported by their two-body Okubo-Zweig-Iizuka allowed strong decay behaviors. In this scheme, we also predict the third radial excitation of the $a_0(980)$, which is denoted as the $a_0(2115)$, accessible at future experiment as a direct test of this assignment. We find another Regge trajectory which contains three isoscalar scalar states $f_0(980)$, $X(1812)$, and $f_0(2100)$. We investigate their two-body Okubo-Zweig-Iizuka allowed strong decay patterns, which are roughly consistent with the experimental data. The $f_0(980)$, $X(1812)$, and $f_0(2100)$ can be well grouped into the isoscalar scalar meson family. We want to emphasize that these two Regge trajectories have a similar slope. In summary, the present work provides a scheme of constructing the scalar meson family based on these reported scalar states. The possibility of the $f_0(1710)$ as the candidate of the scalar glueball cannot be excluded by the observation of the $a_0(1817)$ since the $a_0(1817)$ is more suitable as the isovector partner of the $X(1812)$.

==> Newly observed a_0(1817) as scaling point of constructing scalar meson spectroscopy/figbr.tex <==
\begin{tikzpicture}
\node[below] at (3.85,0.189455) {\scalebox{0.85}{Branching ratios}};
\node[] at (1.3375,4.84763) {\scalebox{0.75}{$\pi\pi$}};
\node[] at (3.0125,4.84763) {\scalebox{0.75}{$\pi\pi(1300)$}};
\node[] at (4.6875,4.84763) {\scalebox{0.75}{$K\bar{K}$}};
\node[] at (6.3625,4.84763) {\scalebox{0.75}{$\eta\eta$}};
\draw[line width=0.50pt,line cap=round] (0.5,2.34027)--(7.2,2.34027);
\draw[line width=0.50pt,line cap=round] (2.175,0.5)--(2.175,4.6406);
\draw[line width=0.50pt,line cap=round] (3.85,0.5)--(3.85,4.6406);
\draw[line width=0.50pt,line cap=round] (5.525,0.5)--(5.525,4.6406);
\draw[] (0.58777,4.55283)--(1.46547,4.55283)--(1.46547,4.01041)--(0.58777,4.01041)--cycle;
\node[] at (1.02662,4.28162) {\scalebox{0.67}{$f_0(1500)$}};
\draw[] (0.58777,2.2525)--(1.46547,2.2525)--(1.46547,1.71008)--(0.58777,1.71008)--cycle;
\node[] at (1.02662,1.98129) {\scalebox{0.67}{$f_0(1370)$}};
\draw[line width=0.50pt,line cap=round] (0.676316,0.5)--(0.676316,0.567);
\node[below] at (0.676316,0.5) {\scalebox{0.75}{0.2}};
\draw[line width=0.50pt,line cap=round] (1.38158,0.5)--(1.38158,0.567);
\node[below] at (1.38158,0.5) {\scalebox{0.75}{0.4}};
\draw[line width=0.50pt,line cap=round] (2.08684,0.5)--(2.08684,0.567);
\node[below] at (2.08684,0.5) {\scalebox{0.75}{0.6}};
\draw[line width=0.50pt,line cap=round] (1.02895,0.5)--(1.02895,0.5335);
\draw[line width=0.50pt,line cap=round] (1.73421,0.5)--(1.73421,0.5335);
\draw[line width=0.50pt,line cap=round] (2.80313,0.5)--(2.80313,0.567);
\node[below] at (2.80313,0.5) {\scalebox{0.75}{0.2}};
\draw[line width=0.50pt,line cap=round] (3.64063,0.5)--(3.64063,0.567);
\node[below] at (3.64063,0.5) {\scalebox{0.75}{0.4}};
\draw[line width=0.50pt,line cap=round] (2.38438,0.5)--(2.38438,0.5335);
\draw[line width=0.50pt,line cap=round] (3.22188,0.5)--(3.22188,0.5335);
\draw[line width=0.50pt,line cap=round] (4.49949,0.5)--(4.49949,0.567);
\node[below] at (4.49949,0.5) {\scalebox{0.75}{0.2}};
\draw[line width=0.50pt,line cap=round] (5.18316,0.5)--(5.18316,0.567);
\node[below] at (5.18316,0.5) {\scalebox{0.75}{0.4}};
\draw[line width=0.50pt,line cap=round] (4.15765,0.5)--(4.15765,0.5335);
\draw[line width=0.50pt,line cap=round] (4.84133,0.5)--(4.84133,0.5335);
\draw[line width=0.50pt,line cap=round] (5.60114,0.5)--(5.60114,0.567);
\node[below] at (5.60114,0.5) {\scalebox{0.75}{0.0}};
\draw[line width=0.50pt,line cap=round] (7.12386,0.5)--(7.12386,0.567);
\node[below] at (7.12386,0.5) {\scalebox{0.75}{0.1}};
\draw[line width=0.50pt,line cap=round] (6.3625,0.5)--(6.3625,0.5335);
\fill[green,opacity=0.5] (1.51558,0.5)--(1.84705,0.5)--(1.84705,4.6406)--(1.51558,4.6406)--cycle;
\fill[green,opacity=0.5] (3.33075,0.5)--(3.55269,0.5)--(3.55269,4.6406)--(3.33075,4.6406)--cycle;
\fill[green,opacity=0.5] (4.06536,0.5)--(4.16791,0.5)--(4.16791,4.6406)--(4.06536,4.6406)--cycle;
\fill[green,opacity=0.5] (6.57568,0.5)--(6.71273,0.5)--(6.71273,4.6406)--(6.57568,4.6406)--cycle;
\draw[line width=0.50pt,line cap=round] (7.2,4.41057)--(7.133,4.41057);
\node[right] at (7.2,4.41057) {\scalebox{0.75}{PDG~\cite{ParticleDataGroup:2020ssz}}};
\draw[line width=0.50pt,line cap=round,gray] (6.37773,4.41057)--(6.65182,4.41057);
\draw[line width=0.50pt,line cap=round,gray] (6.37773,4.34156)--(6.37773,4.47958);
\draw[line width=0.50pt,line cap=round,gray] (6.65182,4.34156)--(6.65182,4.47958);
\fill[red] (6.51477,4.41057)circle(0.0460067);
\draw[line width=0.50pt,line cap=round] (7.2,3.9505)--(7.133,3.9505);
\node[right] at (7.2,3.9505) {\scalebox{0.75}{PDG~\cite{ParticleDataGroup:2020ssz}}};
\draw[line width=0.50pt,line cap=round,gray] (4.07219,3.9505)--(4.14056,3.9505);
\draw[line width=0.50pt,line cap=round,gray] (4.07219,3.88149)--(4.07219,4.01951);
\draw[line width=0.50pt,line cap=round,gray] (4.14056,3.88149)--(4.14056,4.01951);
\fill[red] (4.10638,3.9505)circle(0.0460067);
\draw[line width=0.50pt,line cap=round] (7.2,3.49043)--(7.133,3.49043);
\node[right] at (7.2,3.49043) {\scalebox{0.75}{$\bar{p}d\to 4\pi p$\cite{CRYSTALBARREL:2001ldq}}};
\draw[line width=0.50pt,line cap=round,gray] (2.47755,3.49043)--(3.50139,3.49043);
\draw[line width=0.50pt,line cap=round,gray] (2.47755,3.42142)--(2.47755,3.55944);
\draw[line width=0.50pt,line cap=round,gray] (3.50139,3.42142)--(3.50139,3.55944);
\fill[red] (2.98947,3.49043)circle(0.0460067);
\draw[line width=0.50pt,line cap=round] (7.2,3.03037)--(7.133,3.03037);
\node[right] at (7.2,3.03037) {\scalebox{0.75}{RVUE~\cite{Bugg:1996ki}}};
\draw[line width=0.50pt,line cap=round,gray] (1.20526,3.03037)--(1.93874,3.03037);
\draw[line width=0.50pt,line cap=round,gray] (1.20526,2.96136)--(1.20526,3.09938);
\draw[line width=0.50pt,line cap=round,gray] (1.93874,2.96136)--(1.93874,3.09938);
\fill[red] (1.572,3.03037)circle(0.0460067);
\draw[line width=0.50pt,line cap=round] (7.2,2.5703)--(7.133,2.5703);
\node[right] at (7.2,2.5703) {\scalebox{0.75}{PDG~\cite{ParticleDataGroup:2020ssz}}};
\draw[line width=0.50pt,line cap=round,gray] (1.11005,2.5703)--(1.26521,2.5703);
\draw[line width=0.50pt,line cap=round,gray] (1.11005,2.50129)--(1.11005,2.63931);
\draw[line width=0.50pt,line cap=round,gray] (1.26521,2.50129)--(1.26521,2.63931);
\fill[red] (1.18763,2.5703)circle(0.0460067);
\draw[line width=0.50pt,line cap=round] (7.2,2.11023)--(7.133,2.11023);
\node[right] at (7.2,2.11023) {\scalebox{0.75}{SPEC~\cite{Anisovich:2001ay}}};
\draw[line width=0.50pt,line cap=round,gray] (5.78752,2.11023)--(6.02872,2.11023);
\draw[line width=0.50pt,line cap=round,gray] (5.78752,2.04122)--(5.78752,2.17924);
\draw[line width=0.50pt,line cap=round,gray] (6.02872,2.04122)--(6.02872,2.17924);
\fill[blue] (5.86211,2.06423)rectangle(5.95412,2.15624);
\draw[line width=0.50pt,line cap=round] (7.2,1.65017)--(7.133,1.65017);
\node[right] at (7.2,1.65017) {\scalebox{0.75}{RVUE~\cite{Bugg:1996ki}}};
\draw[line width=0.50pt,line cap=round,gray] (4.56786,1.65017)--(5.45663,1.65017);
\draw[line width=0.50pt,line cap=round,gray] (4.56786,1.58116)--(4.56786,1.71918);
\draw[line width=0.50pt,line cap=round,gray] (5.45663,1.58116)--(5.45663,1.71918);
\fill[blue] (4.96624,1.60416)rectangle(5.05825,1.69617);
\draw[line width=0.50pt,line cap=round] (7.2,1.1901)--(7.133,1.1901);
\node[right] at (7.2,1.1901) {\scalebox{0.75}{$\bar{p}d\to 4\pi p$\cite{CRYSTALBARREL:2001ldq}}};
\draw[line width=0.50pt,line cap=round,gray] (2.29728,1.1901)--(2.65908,1.1901);
\draw[line width=0.50pt,line cap=round,gray] (2.29728,1.12109)--(2.29728,1.25911);
\draw[line width=0.50pt,line cap=round,gray] (2.65908,1.12109)--(2.65908,1.25911);
\fill[blue] (2.43217,1.14409)rectangle(2.52418,1.23611);
\draw[line width=0.50pt,line cap=round] (7.2,0.730033)--(7.133,0.730033);
\node[right] at (7.2,0.730033) {\scalebox{0.75}{RVUE~\cite{Bugg:1996ki}}};
\draw[line width=0.50pt,line cap=round,gray] (0.570526,0.730033)--(1.20526,0.730033);
\draw[line width=0.50pt,line cap=round,gray] (0.570526,0.661023)--(0.570526,0.799043);
\draw[line width=0.50pt,line cap=round,gray] (1.20526,0.661023)--(1.20526,0.799043);
\fill[blue] (0.841888,0.684027)rectangle(0.933901,0.77604);
\draw[line width=0.50pt,line cap=round] (0.5,0.5)--(7.2,0.5)--(7.2,4.6406)--(0.5,4.6406)--cycle;
\end{tikzpicture}

